Data-Driven Offline Optimization For Architecting Hardware Accelerators

Industry has gradually moved towards application-specific hardware accelerators in order to attain higher efficiency. While such a paradigm shift is already starting to show promising results, designers need to spend considerable manual effort and perform a large number of time-consuming simulations to find accelerators that can accelerate multiple target applications while obeying design constraints. Moreover, such a "simulation-driven" approach must be re-run from scratch every time the set of target applications or design constraints change. An alternative paradigm is to use a "data-driven", offline approach that utilizes logged simulation data, to architect hardware accelerators, without needing any form of simulations. Such an approach not only alleviates the need to run time-consuming simulation, but also enables data reuse and applies even when set of target applications changes. In this paper, we develop such a data-driven offline optimization method for designing hardware accelerators, dubbed PRIME, that enjoys all of these properties. Our approach learns a conservative, robust estimate of the desired cost function, utilizes infeasible points, and optimizes the design against this estimate without any additional simulator queries during optimization. PRIME architects accelerators -- tailored towards both single and multiple applications -- improving performance upon state-of-the-art simulation-driven methods by about 1.54x and 1.20x, while considerably reducing the required total simulation time by 93% and 99%, respectively. In addition, PRIME also architects effective accelerators for unseen applications in a zero-shot setting, outperforming simulation-based methods by 1.26x.

==> algorithms/tpo.tex <==
\IncMargin{1.0em}
\begin{algorithm}[t]
\footnotesize
\DontPrintSemicolon
\SetAlgoLined
\SetArgSty{textnormal}
\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{Fppo}{On-Policy}
\SetKwFunction{Fmcts}{TPO}
\For{$\xvar{iteration}\leftarrow$ \scriptsize{1, 2, ..., \xvar{number of iterations}}}{
\If{$\xvar{iteration}\scriptsize{\leq}\rho\;\times$ \xvar{number of iterations}\Comment*[r]{\footnotesize\sffamily\textcolor{black}{\scriptsize{$\textrm{I} \in (0,\;1)$}}}}
{
    $\pi_{c}\:\leftarrow\pi_{(\theta_{old})}$\;
    $L_{c}\:\leftarrow{}L_{\textrm{\supertiny{On-$\pi$}}}^{\textrm{\supertiny{CLIP+VF}}}\scriptstyle (\theta;\phi)$
    %
    \Comment*[r]{\sffamily\textcolor{black}{\scriptsize{On-Policy Training; See Eq.~\ref{eq:l_clip}, \ref{eq:l_vf_clip}, \ref{eq:l_vf}, and \ref{eq:ppo_loss}}}}
}\Else
{
$\pi_{c}\:\leftarrow\pi_{(\theta_{old}; TS)}$\;
\footnotesize{
$L_{c}\:\leftarrow{}L_{\textrm{\supertiny{Off-$\pi$}}}^{\textrm{\supertiny{PF+VF}}}\scriptstyle (\theta;\phi)$\hspace{0.5cm} \Comment*[r]{\footnotesize\sffamily\textcolor{black}{\scriptsize{Off-Policy Training; See Eq.~\ref{eq:l_vf_clip}, \ref{eq:l_vf}, \ref{eq:l_tpo}, and \ref{eq:tpo_loss}}}}}
}
Roll out trajectories \{$\tau_{1}$, $\tau_{2}$, ..., $\tau_{\kappa}$\} for T timesteps each using $\pi_{c}$\;
\For{$\xvar{e}\leftarrow$ \scriptsize{1, 2, ..., \xvar{number of epochs}}}{
Optimize $L_{c}$ wrt to $\theta$ and $\phi$ with minibatch size \xvar{M}\;
}
$\theta_{old}\leftarrow\theta$\;
$\phi_{old}\leftarrow\phi$
}
\caption{\textbf{\benchl{TPO}}\footnotesize{: \textbf{\benchl{T}}ree Search \textbf{\benchl{P}}olicy \textbf{\benchl{O}}ptimization}}
\label{alg:tpo}
\end{algorithm}
\vspace{-0.2cm}
\DecMargin{0.5cm}

==> equations/mean_estimator.tex <==
\begin{equation}
\scalebox{0.9}{$
\mathbf{\hat{\mu}}_{TS}(\textbf{s}_t) = \sum\limits_{k}\frac{N(\textbf{s}_t, \textbf{a}_k)}{N(\textbf{s}_t)}\cdot{\textbf{a}_k}$
%
\label{eq:mean_est}
}
\end{equation}

==> equations/ppo_clipped.tex <==
\begin{equation}
\scalebox{0.9}

     L^{\textrm{CLIP}}(\theta) = \EX_{t}{[\textrm{max}(-\mathfrak{r}_{t}(\theta)\cdot\hat{A}_{t},\; -\textrm{clip}(\mathfrak{r}_{t}(\theta),\;1\;-\;\epsilon,\;1 + \epsilon)\cdot\hat{A}_{t})]};\quad \textrm{where}\quad
     \mathfrak{r}_{t}(\theta) = \frac{\pi_{\theta}(\textbf{a}_t|\textbf{s}_t)}{\pi_{\theta_{old}}(\textbf{a}_t|\textbf{s}_t)}
\label{eq:l_clip}
\end{equation}

==> equations/ppo_loss.tex <==
\begin{equation}
\scalebox{0.9}{$
    L_{\textrm{On-}\pi}^{\textrm{CLIP+VF}}(\theta;\phi) = L^{\textrm{CLIP}}(\theta) + c_{1}\cdot L^{\textrm{VF}}(\phi)$
%
    \label{eq:ppo_loss}
}
\end{equation}

==> equations/q_function.tex <==
\vspace{-0.2cm}
\begin{equation}
\scalebox{0.9}

Q(\textbf{s}_t, \textbf{a}_k) = \textrm{r}(\textbf{s}_t, \textbf{a}_k) + \gamma \frac{W(\textbf{s}_t, \textbf{a}_k)}{N(\textbf{s}_t, \textbf{a}_k)}
\label{eq:q_func}
\end{equation}

==> equations/tpo_loss.tex <==
\begin{equation}
\scalebox{0.9}{$
    L_{\textrm{Off-}\pi}^{\textrm{PF+VF}}(\theta;\phi) = L^{\textrm{PF}}(\theta) + c_{3}\cdot L^{\textrm{VF}}(\phi)$
%
\label{eq:tpo_loss}
}
\end{equation}

==> equations/tpo_policy_loss.tex <==
\begin{equation}
\scalebox{0.9}
     L^{\textrm{PF}}(\theta) = \EX_{t}[(\mathbf{\hat{\mu}}_{\mathrm{TS}}(\textbf{s}_t) - \mathbf{\mu}_{\pi_{\theta}}(\textbf{s}_t))^2 + c_2\cdot(\mathbf{\hat{\sigma}}_{\mathrm{TS}}(\textbf{s}_t) - \mathbf{\sigma}_{\pi_{\theta}}(\textbf{s}_t))^2]
\label{eq:l_tpo}
\end{equation}

==> equations/u_function.tex <==
\vspace{-0.2cm}
\begin{equation}
\scalebox{0.9}

U(\textbf{s}_t, \textbf{a}_k) = \textrm{c}_{puct} \cdot \pi_{\theta}(\textbf{a}_k|\textbf{s}_t)\cdot\frac{\sqrt{N(\textbf{s}_t)}}{1 + N(\textbf{s}_t, \textbf{a}_k)}
\label{eq:u_func}
\end{equation}

==> equations/value_loss.tex <==
\vspace{-0.1cm}
\begin{equation}
\scalebox{0.9}
     V_{\phi}^{\textrm{CLIP}}(\textbf{s}_t) = V_{\phi_{old}}(\textbf{s}_t) + \textrm{clip}(V_{\phi}(\textbf{s}_t) - V_{\phi_{old}}(\textbf{s}_t), -\epsilon,  \;\;\epsilon)
\label{eq:l_vf_clip}
\end{equation}
\vspace{-0.2cm}
\begin{equation}
\scalebox{0.9}{
$L^{\textrm{VF}}(\phi) = \EX_{t}[\textrm{max}((V_{\phi}^{\textrm{CLIP}}(\textbf{s}_t) - V_{t}^{targ})^2,\;\;(V_{\phi}(\textbf{s}_t) - V_{t}^{targ})^2)]$
\label{eq:l_vf}
}
\end{equation}

==> tables/benchmark.tex <==
\begin{table}
\vspace{-0.3cm}
\small
\begin{center}
\begin{tabular}{ |l|l|l| }\hline
Environments & State Space & Action Space \\
\hline\hline 
\bench{Ant-v2} & $\mathbb{R}^{111}$ & $[-1.0, 1.0]^{8}$\\
\bench{HalfCheetah-v2} & $\mathbb{R}^{17}$ & $[-1.0, 1.0]^{6}$\\
\bench{Hopper-v2} & $\mathbb{R}^{11}$ & $[-1.0, 1.0]^{3}$\\
\bench{Humanoid-v2} & $\mathbb{R}^{376}$ & $[-0.4, 0.4]^{17}$\\
\bench{Swimmer-v2} & $\mathbb{R}^{8}$ & $[-1.0, 1.0]^{2}$\\
\bench{Walker2d-v2} & $\mathbb{R}^{17}$ & $[-1.0, 1.0]^{6}$\\\hline
\end{tabular}
\caption{The benchmark suite (six OpenAI Gym~\cite{openaigym:arxiv:16} environments) with their corresponding observation/action spaces.}
\label{table:benchmarks}
\end{center}
\vspace{-0.7cm}
\end{table}

==> tables/dataset.tex <==
\bgroup
\def\arraystretch{1.0}
\setlength\tabcolsep{2.0pt}
\begin{table*}[ht]
\scriptsize
  \begin{center}
    \caption{Total number of feasible and infeasible data points available in the dataset out of 452,760,000 data points in the search space. The last column shows the maximum number of data used for training the surrogate model (large dataset).}
    \label{tab:ds}
    \begin{tabular}{@{}l|l|l|l@{}}
    \textbf{Name}&\textbf{\# of Feasible}&\textbf{\# of Infeasible}&\textbf{\# of Feasible in Training (large)}\\
    \hline
    MobileNetEdge~\cite{efficientnet:2020}&115,711&384,355&13,482\\
    MobileNetV2~\cite{mnv2:arxiv:2018}&127,707&372,359&13,083\\
    MobileNetV3~\cite{mnv3:cvpr:2019}&101,336&398,730&12,018\\
    \mfour&104,074&395,992&13,564\\
    \mfive&150,757&349,309&19,468\\
    \msix&121,832&378,234&12,063
    \end{tabular}
  \end{center}
\end{table*}
\egroup

==> tables/feasibility_ratio.tex <==
\begin{table}[htbp]
  \begin{center}
    \caption{The average feasibility and uniqueness ratio across five runs for architecture search with an area budget of 6.8 $\mathrm{mm^2}$ (see Figure~\ref{fig:va_6.8}).}
    \label{tab:feas_ratio}
    \begin{tabular}{l||c|c|c|c|c}
      & \bench{Evolutionary} & \bench{MBO} & \bench{P3BO} & \bench{Random} & \bench{Vizier}\\
      \hline
      Avg. Feasibility Ratio ($\uparrow$ better)	& 0.362 & 0.803 & 0.347 & 0.009 & 0.012 \\
      Avg. Uniqueness Ratio ($\uparrow$ better) & 0.891 & 0.236 & 0.848 & 1.0 & 0.979
    \end{tabular}
  \end{center}
\end{table}

% Feasibility
% Evolutionary    0.362305
% MBO             0.803516
% P3BO            0.346924
% Random          0.008740
% Vizier          0.012305

% uniqueness
% Evolutionary    0.891211
% MBO             0.235645
% P3BO            0.848291
% Random          1.000000
% Vizier          0.979102

==> tables/ppo-hyperparam.tex <==
% \begin{table}
% \caption{\small{\bench{TPO}/\bench{PPO} hyperparameters used to evaluate \muj-simulated environments on a \benchl{2$\times$2-TPU~v2}. We adjust the hyperparameters to replicate the reported \bench{PPO} results with our infrastructure setup.}}
% \vspace{2pt}
% \small
% \begin{center}
% \begin{tabular}{ l|c }\hline
%  Hyperparameters & Value  \\ 
%  \hline\hline 
%  \bench{Policy network architecture} & \bench{FC:64 -- FC:64}\\
%  \bench{Value network architecture} & \bench{FC:64 -- FC:64}\\
%  \bench{Adam stepsize ($\eta$)} & \xxs{3}\xxs{$\times\textrm{10}^{\textrm{-4}}$} and  \xxs{9}\xxs{$\times\textrm{10}^{\textrm{-4}}$}\\
%  \bench{Horizon (T)} & \xxs{2048}\\
%  \bench{Switching ratio ($\rho$)} & \xxs{0.5}\\
%  \bench{Clipping coefficient ($\epsilon$)} & \xxs{0.2}\\
%  \bench{Number of epochs} & \xxs{10}\\
%  \bench{Minibatch size (M)} & \xxs{128}\\
%  \bench{Gradient norm clipping coefficient} & \xxs{0.5}\\
%  \bench{Discount ($\gamma$)} & \xxs{0.99}\\
%  \bench{GAE parameter ($\lambda$)} & \xxs{0.95}\\
% \hline
% \end{tabular}
% \end{center}
% \label{table:ppo_hparams}
% \vspace{-0.5cm}
% \end{table}
\setlength\intextsep{1pt}
\setlength{\columnsep}{4pt}%
\begin{wraptable}[22]{r}{0.53\textwidth}
  \begin{center}
\caption{\tpo hyperparameters.}
\vspace{-0.2cm}
%\quad
\begin{tabular}{ |l|c| }\hline
\footnotesize{MCTS Hyperparameters} & \footnotesize{Value}  \\ 
 \hline\hline 
 \bench{Number of MCTS simulations} & \bench{32}\\
 \bench{Maximum number of actions per node} & \bench{32}\\
 \bench{c$_{\textrm{puct}}$} & \bench{3}\\
 \bench{Temperature ($\tau$)} & \bench{5}\\
 \bench{Dirichlet noise scaling parameter ($\alpha$)} & \bench{1.75}\\
  \bench{Dirichlet noise weight ($\omega$)} & \bench{0.5}\\
  \hline\hline
  \footnotesize{Training Hyperparameters} & \footnotesize{Value}\\ 
  \hline\hline
  \bench{Policy network architecture} & \bench{FC:64 -- FC:64}\\
 \bench{Value network architecture} & \bench{FC:64 -- FC:64}\\
 \bench{Adam learning rate ($\eta$)} & \xxs{3}\xxs{$\times\textrm{10}^{\textrm{-4}}$} and  \xxs{9}\xxs{$\times\textrm{10}^{\textrm{-4}}$}\\
 \bench{Horizon (T)} & \xxs{2048}\\
 \bench{Switching ratio ($\rho$)} & \xxs{0.5}\\
 \bench{Clipping coefficient ($\epsilon$)} & \xxs{0.2}\\
 \bench{Number of epochs} & \xxs{10}\\
 \bench{Minibatch size (M)} & \xxs{128}\\
 \bench{Gradient norm clipping coefficient} & \xxs{0.5}\\
 \bench{Discount ($\gamma$)} & \xxs{0.99}\\
 \bench{GAE parameter ($\lambda$)} & \xxs{0.95}\\
\hline
\end{tabular}
\label{table:hparams}
\end{center}
\end{wraptable}

==> tables/results.tex <==
\begin{table}[!b]
\vspace{-0.5cm}
\caption{Performance comparison between \protect{\bench{\tpo}} and \protect{\bench{PPO}} after \xxs{4M} time-steps. $\Delta$ values show the difference between \tpo and PPO for each category. A positive $\Delta$ value indicates that TPO outperforms PPO.
}
\vspace{-0.3cm}
\footnotesize
\begin{center}
{
\setlength\tabcolsep{1.5pt}
\begin{tabular}{|l|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|P{1.2cm}|}\hline
 \multirow{2}{*}{Benchmarks}& \multicolumn{3}{|c|}{\textbf{Min.}}&\multicolumn{3}{|c?}{\textbf{Avg.}}&\multicolumn{3}{|c|}{\textbf{Max.}}\\
 \cline{2-10}
 & PPO & \tpo & $\Delta$ & PPO & \tpo & $\Delta$ & PPO & \tpo & $\Delta$ \\
\hline\hline

\bench{Ant-v2} & \xxs{1722.75} & \xxs{{4455.57}} & \xxs{$+$2732.81} &\xxs{1873.85} & \xxs{{4777.06}} & \xxs{$+$2903.21} &\xxs{2022.08} & \xxs{{5011.08}} & \xxs{$+$2989.0}\\
 
 \bench{HalfCheetah-v2} & \xxs{1658.70} & \xxs{{1788.77}} & \xxs{$+$130.06} & \xxs{2530.81} & \xxs{{3949.05}} & \xxs{$+$1418.24} & \xxs{5049.07} & \xxs{{6734.45}} &\xxs{$+$1685.38} \\
 
 \bench{Hopper-v2} & \xxs{1744.24} & \xxs{{2205.47}} &\xxs{$+$461.22}& \xxs{1937.82} & \xxs{{3196.14}}  &\xxs{$+$1258.32}& \xxs{2051.89} & \xxs{{3613.36}}&\xxs{$+$1561.47}\\
 
 \bench{Humanoid-v2} & \xxs{4269.44} & \xxs{{5391.43}}  &\xxs{$+$1121.99}& \xxs{4439.58} &  \xxs{{5460.93}}&\xxs{$+$1021.35} & \xxs{4609.72} & \xxs{{5530.43}} & \xxs{$+$920.71}\\
 
 \bench{Swimmer-v2} & \xxs{109.91} & \xxs{{119.48}} &\xxs{$+$9.57}& \xxs{113.74} & \xxs{{120.81}} &\xxs{$+$7.07}& \xxs{116.74} & \xxs{{122.39}}&\xxs{$+$5.65}\\
 
 \bench{Walker2d-v2} & \xxs{3605.27} & \xxs{{3788.83}} &\xxs{$+$183.56}& \xxs{3942.57} & \xxs{{4092.21}} &\xxs{$+$149.63}& \xxs{4155.37} & \xxs{{4667.64}}&\xxs{$+$512.27}\\
 
 \hline
\end{tabular}}
\end{center}
\vspace{-0.3cm}
\label{table:summary:results}
\end{table}
